Bias Mimicking: A Simple Sampling Approach for Bias Mitigation

Prior work has shown that Visual Recognition datasets frequently underrepresent bias groups $B$ (\eg Female) within class labels $Y$ (\eg Programmers). This dataset bias can lead to models that learn spurious correlations between class labels and bias groups such as age, gender, or race. Most recent methods that address this problem require significant architectural changes or additional loss functions requiring more hyper-parameter tuning. Alternatively, data sampling baselines from the class imbalance literature (\eg Undersampling, Upweighting), which can often be implemented in a single line of code and often have no hyperparameters, offer a cheaper and more efficient solution. However, these methods suffer from significant shortcomings. For example, Undersampling drops a significant part of the input distribution per epoch while Oversampling repeats samples, causing overfitting. To address these shortcomings, we introduce a new class-conditioned sampling method: Bias Mimicking. The method is based on the observation that if a class $c$ bias distribution, \ie $P_D(B|Y=c)$ is mimicked across every $c^{\prime}\neq c$, then $Y$ and $B$ are statistically independent. Using this notion, BM, through a novel training procedure, ensures that the model is exposed to the entire distribution per epoch without repeating samples. Consequently, Bias Mimicking improves underrepresented groups' accuracy of sampling methods by 3\% over four benchmarks while maintaining and sometimes improving performance over nonsampling methods. Code: \url{https://github.com/mqraitem/Bias-Mimicking}

==> 8_ethics_rep.tex <==
\noindent\textbf{Code of Ethics Statement} Our work addresses a critical problem within the fairness literature: spurious predictive behavior by Deep Learning models. We measure this behavior by calculating the dataset's subgroups' predictive performance (accuracy). While this metric aligns with our goal of measuring and preventing spurious behavior, we emphasize that the metric is not exhaustive of other fairness concerns. We refer the reader to \cite{impossible-fair} for a broader discussion of fairness metrics. Furthermore, while our proposed method aims to learn robust representations for underrepresented subgroups within a given dataset, we acknowledge that such representations could be misused in downstream applications that could raise ethical concerns (\eg surveillance). Furthermore, two of the datasets used in our experiments involve facial attribute recognition tasks (\eg hair color). Models trained on these datasets could be misused, yet they remain standard benchmarks for evaluating spurious correlations. We encourage future researchers and practitioners to use this technology with care and caution. 

\noindent\textbf{Reproducibility Statement}
We provide the source code for this work in the supplementary. The training and hyper-parameters to reproduce the results are outlined in Appendix \ref{sec:hyper-model-details-supp}. Moreover, The results we report in this paper were averaged over 3 runs with different seeds, and standard deviations were reported to ensure statistical significance. Furthermore, all experiments were done on datasets that are publicly available online. 
